Nonparametric estimation of a multivariate density under Kullback-Leibler loss with ISDE

In this paper, we propose a theoretical analysis of the algorithm ISDE, introduced in previous work. From a dataset, ISDE learns a density written as a product of marginal density estimators over a partition of the features. We show that under some hypotheses, the Kullback-Leibler loss between the proper density and the output of ISDE is a bias term plus the sum of two terms which goes to zero as the number of samples goes to infinity. The rate of convergence indicates that ISDE tackles the curse of dimensionality by reducing the dimension from the one of the ambient space to the one of the biggest blocks in the partition. The constants reflect a combinatorial complexity reduction linked to the design of ISDE.

==> GANs.tex <==
\section{Approximation term with GANs}

In this appendix, we present another path to control the approximation term with vanilla Generative Adversarial Network. This problem was recently studied in \cite{belomestny2021rates}.  Their results require stronger assumptions than what is presented in the paper, in particular that the statistician knows the constant $A$ involved in condition (BC). What is more, 

\subsection{Regularity conditions}

\paragraph{Bounding condition} Density estimation under Kullback-Leiber loss is known to be a challenging problem. One work by \cite{hall1987kullback} has studied the asymptotic convergence rates for kernel estimators in a one-dimensional setting. It was shown that the tails of the kernel must be chosen appropriately regarding the tails property of the proper density to have convergent estimators. Thought theoretically relevant, these results are of poor interest for the practitioner who does not have this kind of information about the true density.

In this work, we choose to restrict our attention to densities that are lower and upper bounded by some positive quantities. This is done to avoid hardly tractable tail behavior issues. In the sequel we consider that the following bounding condition is true for all $S \in \Sdk$  :

\begin{equation}
    \tag{BC}
    \left\{
    \begin{array}{l}
       e^{-A |S|} \leq f_S \leq e^{A |S|} \ \forall S \in \Pstar \\
    \end{array}
    \right.
    \label{BC}
\end{equation}

Fulfilling the condition implying $\hat{f}$ requires that $A$ is known by the statistician and can be used in estimation procedure. Under \ref{BC} it can be shown that the Kullback-Leibler loss can be controlled by the Jensen-Shannon ($\mathrm{JS}$) loss defined as follows
\begin{equation}
    \JS{f}{g} = \frac{1}{2}\KL{f}{\frac{f+g}{2}} + \frac{1}{2}\KL{g}{\frac{f+g}{2}}.
\end{equation}

\begin{myprop}{Control of KL by JS}{controlKLJS}
Under \ref{BC}, for any $S \in \Pstar$ :
\begin{equation}
    \KL{f_S}{\hat{f}_S} \leq \frac{8(1 + A|S|)}{2 \log 2 - 1}\JS{f_S}{\hat{f}_S}.
\end{equation}
\end{myprop}

\begin{proof}
Lemma 7.23 in \cite{massart2007concentration} ensures that 
\begin{equation}
    \KL{f_S}{\hat{f}_S} \leq \frac{4(1 + A|S|)}{2 \log 2 - 1}\KL{f_S}{\frac{\hat{f}_S + f_S}{2}}
\end{equation}
Then, using the nonnegativeness  of $\mathrm{KL}$, we obtain
\begin{equation}
    \KL{f_S}{\hat{f}_S} \leq \frac{8(1 + A|S|)}{2 \log 2 - 1}\left( \frac{1}{2}\KL{f_S}{\frac{\hat{f}_S + f_S}{2}} + \frac{1}{2}\KL{\hat{f}_S}{\frac{\hat{f}_S + f_S}{2}} \right).
\end{equation}
\end{proof}

\cite{belomestny2021rates} obtained result on the convergence rate for density estimation under JS loss. The lemma above demonstrates that their results could also be applied in our context under \ref{BC}.
 
\paragraph{$A$-regular Hölder ball} Let $p$ and $q$ be a positive integer and $g : [0, 1]^p \rightarrow [0, 1]^q$ a function. Let $\gamma = (\gamma_1, \dots, \gamma_p) \in \mathbb{N}^d$ be a multiindex and let $|\gamma| = \sum_{i = 1}^p \gamma_i$ be its order. The partial differentiate operator $D^\gamma$ is defined as follows
\begin{equation}
    \forall i \in \{1, \dots, q\}, \ D^\gamma g_i = \frac{\partial^{|\gamma|} g_i}{\partial^{\gamma_i}_{x_1} \dots \partial^{\gamma_d}_{x_d}}.
\end{equation}

For a positive number $\alpha$, if we denote by $s$ the larger integer strictly lower than $\alpha$ and let $\delta = \alpha - s \in (0, 1]$, $g$ belongs to the Hölder ball $\mathcal{H}^\alpha(p, q, H)$ where $H$ is a positive real number if both following conditions are fullfilled

\begin{equation}
    \left\{
    \begin{array}{l}
        \underset{|\gamma | \leq s}{\max}\ \  \underset{1 \leq i \leq q}{\max}\ \  \underset{x \in [0, 1]^p}{\sup} \  \Vert D^\gamma g_i(x) \Vert \leq H \\
        \underset{|\gamma | = s}{\max}\ \  \underset{1 \leq i \leq q}{\max}\ \  \underset{x, y \in [0, 1]^p}{\sup} \  \frac{\left| D^\gamma g_i(x) - D^\gamma g_i(y) \right|}{\Vert x-y\Vert ^\delta} \leq H.
    \end{array}
    \right.
\end{equation}

Moreover, for $A > 0$, $g$ belongs to the $A$-regular Hölder ball $\mathcal{H}_A^\alpha(p, q, H)$ if $g \in \mathcal{H}^\alpha(p, q, H)$ and for all $x \in [0, 1]^p$
\begin{equation}
    e^{-2 A} I_q \preccurlyeq \nabla g(x)^{\mathrm{T}} \nabla g(x) \preccurlyeq e^{2 A} I_q
\end{equation}
where $\nabla g$ is the Jacobian and where for symmetric matrices $M$ and $N$, $N \preccurlyeq M$ means that $M-N$ is positive. This condition implies in particular that $g$ is invertible.

\subsection{Assumptions on the true density}\label{AssumptionTrueDensity}

We will consider regularity condition on the true density of a particular form. Let $g$ be a function from $[0, 1]^p$ to $[0, 1]^p$, invertible and such as for all $x \in [0, 1]^p$, $\det \nabla g(x) \neq 0$. It is possible to define a density $t$ over $[0, 1]^p$ as the density of the random variable $g(U)$ where $U$ is uniformly distributed over $[0, 1]^p$ with the following formula
\begin{equation}
    \forall x \in [0, 1]^p, \ t(x) = \frac{1}{\left| \det \nabla g (g^{-1}(x)) \right|}.
\end{equation}

Let us now formulate the regularity condition for $(f_S)_{S \in \Pstar}$. Let $A > 0, \beta > 0$ and $H > 0$, we assume that for all $S \in \Pstar$, it exists $g_S \in \mathcal{H}_A^{1 + \beta}(|S|, |S|, H)$ such that for all $x_S \in [0, 1]^{|S|}$
\begin{equation}
    f_S(x_S) = \frac{1}{\left| \det \nabla g_S (g_S^{-1}(x_S)) \right|}.
\end{equation}

The assumption that $g_S$ is $A$-regular implies that for all $x_S \in [0, 1]^{|S|}$, $e^{-A|S|} \leq \det \nabla g_S(x_s) \leq e^{A|S|}$ and then that the formula above is well defined and that  $e^{-A|S|} \leq f_S(x_s) \leq e^{A|S|}$, proving that \ref{BC} is satisfied for the true density.

\subsection{Choice of multidimensional estimators}

\paragraph{Neural Networks} Let $p$ and $q$ be two positive integer. A neural network (NN) is a function $\mathbb{R}^p \rightarrow \mathbb{R}^q$ enjoying a particular structure. Let $\sigma : \mathbb{R} \rightarrow \mathbb{R}$ be a nonlinear function called activation function. Famous examples are ReLu : $\sigma_\text{ReLu}(x) = x \mathbb{1}_{[0, + \infty]}(x)$ or ReQu : $\sigma_\text{ReQu}(x) = x^2 \mathbb{1}_{[0, + \infty]}(x)$. Different architectures of NNs exist, we focus here on densely connected networks.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.5]{relurequ.png}
    \caption{ReQu and ReLu activation functions}
    \label{fig:relurequ}
\end{figure}

A NN encodes a function $f_\text{NN}$ which is a composition of linear operation and nonlinear operations :
\begin{equation}
    f_\text{NN} = W_{L+1} \circ \phi \circ W_L \circ \phi \circ \dots \circ \phi \circ W_1.
\end{equation}

$L$ is the number of hidden layer and the shape of the network is determined by a vector $\ell = (l_1, \dots, l_L)$ corresponding to the dimension of each hidden layer. Each $W_i$ represent an affine function $W_i = A_ix + b_i$ taking values in $\mathbb{R}^{l_i}$ with the convention that $l_{L+1} = q$ and $\phi$ as a multidimensional function with a slight abuse of notation. If $x \in \mathbb{R}^r$, $\phi(x) = \left(\phi(x_1), \dots, \phi(x_r)\right)^\mathrm{T}$. We denote by $\text{NN}_{(p, q)}$ the set of all neural nets with input dimension $p$ and output dimension $q$.

It is natural to represent a neural net as an oriented graph, as in the figure below.

\begin{figure}[ht]
\centering
\begin{neuralnetwork}[height=4]
    \newcommand{\x}[2]{$x_#2$}
    \newcommand{\y}[2]{$\hat{y}_#2$}
    \newcommand{\hfirst}[2]{\small $h^{(1)}_#2$}
    \newcommand{\hsecond}[2]{\small $h^{(2)}_#2$}
    \inputlayer[count=3, bias=false, title=Input\\layer]
    \hiddenlayer[count=4, bias=false, title=Hidden\\layer 1] \linklayers
    \hiddenlayer[count=3, bias=false, title=Hidden\\layer 2] \linklayers
    \outputlayer[count=2, title=Output\\layer] \linklayers
\end{neuralnetwork}
\label{GraphNN}
\caption{Graphical representation of a NN with $p=3$, $q=2$, $L=2$, $\ell = (4, 3)$}
\end{figure}

We define a restricted class of NNs, where we impose the maximal coefficient involved in affine operations to be smaller than one, and we restrict the number of non-zero coefficients.

\begin{equation}
    \begin{split}
        \text{NN}_{(p, q)}\left(L, \ell, s\right) = \{ f_{\text{NN}} \in \text{NN}_{(p, q)}\ \left| &\max_{i=1, \dots, L+1} \left\Vert A_i  \right\Vert_\infty \vee \left\Vert b_i \right\Vert_\infty \leq 1 \\
        &\text{and} \ \sum_{i=1, \dots L+1} \Vert A_i \Vert_0 + \Vert b_i \Vert_0 \leq s \right. \}.
    \end{split}
\end{equation}

\paragraph{GANs} Generative Adversarial Networks (GANs) were introduced in \cite{goodfellow2014generative}. The principle is to design an algorithm able to generate fake data hardly distinguishable from an input data sample and implicitly acquire knowledge about the underlying distribution. It has become a prevalent tool in artificial intelligence. Remarkable realizations based on the use of GANs include generating realistic photographs of human faces (\cite{karras2017progressive}), performing vector arithmetic in natural images space  (\cite{radford2015unsupervised}) or video prediction (\cite{vondrick2016generating}).

Assume that we have at our disposal a $n$-sample $A_1, \dots, A_n$ drawn independently from a probability density $t$ over $\mathcal{A} \subset \mathbb{R}^p$. A GAN is composed by two elements: a discriminator $D$ and a generator $G$.

\begin{itemize}
    \item The discriminator $D$ is a function from $\mathcal{A}$ to $[0, 1]$ aimed to discriminate data coming from $t$ to other distribution.
    \item The generator $G$ is used to generate fake data. Given a probability density $\phi$ over $\mathbb{R}^{p'}$ where $p'$ can be any integer (we can restrict ourselves to the case where $\phi$ is uniform over $[0,1]^{p'}$) and a point $y$ drawn from $\phi$, $G(y)$ is a fake data point in $\mathcal{A}$.
\end{itemize}

The objective is to produce a generator that makes the discriminator unable to distinguish between real and fake samples. Given a family of discriminators $\mathcal{D}$ and a family of generators $\mathcal{G}$ the optimization problem introduced by \cite{goodfellow2014generative} and referred to as vanilla GAN is

\begin{equation}
    \min_{G \in \mathcal{G}} \max_{D \in \mathcal{D}} \left\{ L(G, D) = \frac{1}{2} \mathbb{E}_{A \sim t} \left[ \log(D(A)) \right] + \frac{1}{2} \mathbb{E}_{Y \sim \phi} \left[ \log(1 -D(G(Y))) \right] \right\}.
\end{equation}

If $Y_1, \dots, Y_n$ is a $n$-sample drawn independently from $\phi$, the corresponding empirical optimization problem is 

\begin{equation}
    \min_{G \in \mathcal{G}} \max_{D \in \mathcal{D}} \left\{ L_n(G, D) = \frac{1}{2} \sum_{i=1}^n \log(D(A_i)) + \frac{1}{2} \sum_{i=1}^n \log(1 - D(G(Y_i)))\right\}.
    \label{eq:empiricalGANformulation}
\end{equation}

In what follows we will consider that take $\mathcal{D}$ and $\mathcal{G}$ as subsets of, respectively $\text{NN}_{(p, 1)}$ and $\text{NN}_{(p, p)}$. 

\paragraph{From neural network to density}

GANs are tools to construct networks allowing to sample from an unknown distribution. In our context we need to be able to extract from the generator $G$ a density function $\hat{t}$ over $\mathcal{A}$. We assume here that $p' = p$ and that $\phi$ is the uniform distribution over $[0, 1]^p$. Then $G(Y)$ is a random variable admitting $\hat{t}$ as density function. Following what we have presented in \cref{AssumptionTrueDensity}, under suitable conditions on $G$, $\hat{t}$ can be written as follows 
\begin{equation}
    \forall x \in \mathcal{A}, \hat{t}(x) = \frac{1}{\left| \det \nabla G (G^{-1}(x)) \right|}.
    \label{fromNNtodensity}
\end{equation}


\paragraph{Choice of $\mathcal{D}$ and $\mathcal{G}$} In order to use ISDE, we need to define a family of marginal density estimators $(\hat{f}_S)_{S \in \Sdk}$. To do so we train a family of GANs $\left(\mathcal{G}_S, \mathcal{D}_S \right)_{S \in \Sdk}$, on data $W_1, \dots, W_m$ by solving \ref{eq:empiricalGANformulation}, and extract density estimators $\hat{f}$. We will impose the following conditions on $\mathcal{D}_S$ and $\mathcal{G}_S$. It exists $L_S^\mathcal{G}, l_S^\mathcal{G}, s^\mathcal{G}_S \text{ and } H_S^\mathcal{G}$ such that
\begin{equation}
    \mathcal{G}_S = \text{NN}_{(|S|, |S|)}\left(L_S^\mathcal{G}, \ell_S^\mathcal{G}, s_S^\mathcal{G}\right) \cap \mathcal{H}^2_{2A}\left( |S|, |S|,  H_S^{\mathcal{G}} \right).
\end{equation}
Similarly, it exists $L_S^\mathcal{D}, l_S^\mathcal{D}, s^\mathcal{D}_S \text{ and } H_S^\mathcal{D}$ such that 
\begin{equation}
    \mathcal{D}_S = \text{NN}_{(|S|, 1)}\left(L_S^\mathcal{D}, \ell_S^\mathcal{D}, s_S^\mathcal{D}\right) \cap \mathcal{H}^1\left( |S|, 1, H_S^{\mathcal{D}} \right).
\end{equation}
Moreover we assume that there exists $0 < D_\text{min} < D_\text{max} < 1$ such that for all $D_S \in \mathcal{D}_S$ and for all $x \in [0, 1]^{|S|}$, $D_S(x) \in [D_\text{min}, D_\text{max}]$.

The condition that $\hat{f}_S$ must be $2A$-regular ensures that \cref{BC} is satisfied for $(\hat{f}_S)_{S \in Pdk}$, with the same reasoning as the one presented in \cref{AssumptionTrueDensity}.

\subsection{Rate of convergence}

With the previously introduced notations, we can state the following theorem, which is valid under a good choice of constants involved in the definitions of $\left(\mathcal{G}_S\right)_{S \in \Pstar}$ and $\left(\mathcal{D}_S\right)_{S \in \Pstar}$, and which is a direct application of Theorem 2 in \cite{belomestny2021rates}.

\begin{mythm}{Convergence rate for the approximation term}{rateconvergenceapproximatio}

\begin{equation}
    \esperance{\sum_{S_* \in \Pstar} \KL{f_S}{\hat{f_S}}} \lesssim \left(\frac{\log m}{m}\right)^{\frac{2 \beta}{2 \beta + \underset{S \in \Pstar}{\max} |S|}}.
\end{equation}
And, as $\underset{S \in \Pstar}{\max} |S| \leq k$
\begin{equation}
    \esperance{\sum_{S_* \in \Pstar} \KL{f_S}{\hat{f_S}}} \lesssim \left(\frac{\log m}{m}\right)^{\frac{2 \beta}{2 \beta + k}}.
\end{equation}
\end{mythm}

The convergence rate depends on the regularity parameter $\beta$ and the parameter $k$. Its dependence in $k$ highlights how ISDE tackles the curse of dimensionality. Considering no independence structure would lead to a similar convergence speed, but where $k$ is replaced by $d$. Here the smaller $k$, the faster the approximation term converges.

